Message Passing Neural Processes

Neural Processes (NPs) are powerful and flexible models able to incorporate uncertainty when representing stochastic processes, while maintaining a linear time complexity. However, NPs produce a latent description by aggregating independent representations of context points and lack the ability to exploit relational information present in many datasets. This renders NPs ineffective in settings where the stochastic process is primarily governed by neighbourhood rules, such as cellular automata (CA), and limits performance for any task where relational information remains unused. We address this shortcoming by introducing Message Passing Neural Processes (MPNPs), the first class of NPs that explicitly makes use of relational structure within the model. Our evaluation shows that MPNPs thrive at lower sampling rates, on existing benchmarks and newly-proposed CA and Cora-Branched tasks. We further report strong generalisation over density-based CA rule-sets and significant gains in challenging arbitrary-labelling and few-shot learning setups.

==> old_tables.tex <==

\begin{table}
  \scriptsize
  \caption{Node classification on biochemical datasets. Accuracy reported at $\{5, 10, 30\}$\% context points. {\ubold first} / {\usecond second}.}
  \label{t:node-tu}
  \centering
  \resizebox{\textwidth}{!}{\begin{tabular}{lccc|ccc|ccc|ccc|ccc}
    \toprule
    & \multicolumn{3}{c}{Proteins} & \multicolumn{3}{c}{Enzymes} & \multicolumn{3}{c}{DHFR} & \multicolumn{3}{c}{COX2} & \multicolumn{3}{c}{BZR} \\
    Model & 5 & 10 & 30 & 5 & 10 & 30 & 5 & 10 & 30 & 5 & 10 & 30 & 5 & 10 & 30 \\
    \midrule
    NP       & 66.24&81.51&\usecond93.62 & \usecond79.23 &93.43&\usecond95.75 & 54.66&55.71&57.38 & 79.35&81.05&81.54 & 61.35&61.28&61.89 \\
    NP-c     & 65.16&79.72&92.10 & 78.02&92.64&94.94 & 54.51&56.35&56.20 & 76.81&77.52&77.29 & 60.62&61.17&60.62 \\
    \midrule
    MPNP     & 65.58&80.55&91.78 & 79.09&\usecond94.10&\ubold95.78 & 88.65&89.62&90.53 & 89.99&89.89&90.27 &  \usecond89.59&\usecond89.80&\usecond90.22 \\
    MPNP-c   & \usecond 66.96& \usecond 82.28&\ubold94.18 & 79.02&93.91&95.65 & \usecond89.29&\usecond89.75&\usecond90.83 &  \usecond90.00&\usecond91.37&\usecond91.94 & 88.34&88.72&88.77 \\
    \midrule
    GCN      & \ubold87.37 & \ubold87.37 & 87.37 & \ubold94.23 &\ubold 94.23 & 94.23&\ubold 93.35 &\ubold 93.35 &\ubold 93.35 &\ubold 94.92 &\ubold 94.92 &\ubold 94.92 &\ubold 97.93 &\ubold 97.93 &\ubold 97.93 \\
    \texttt{labelprop}     & 59.52&63.15&74.44 & 58.93&63.91&76.42 & 38.48& 41.51&53.63 & 39.43&42.42&57.08 & 40.77&44.54&57.08 \\
    \bottomrule
  \end{tabular}}
\end{table}

\begin{table*}
  \scriptsize
  \caption{ShapeNet mixed-class results. We report the mIoU for $\{0.1, 1, 5, 10, 30\}$\% context points.}
  \label{t:node-shapenetmixed}
  \centering
  \resizebox{\textwidth}{!}{\begin{tabular}{lccccc|ccccc|ccccc}
    \toprule
     & \multicolumn{5}{c}{2-class} & \multicolumn{5}{c}{3-class} & \multicolumn{5}{c}{4-class} \\
     Model & 0.1 & 1 & 5 & 10 & 30 & 0.1 & 1 & 5 & 10 & 30 & 0.1 & 1 & 5 & 10 & 30 \\
    \midrule
    NP-c     & 48.06&83.60&88.61&89.17&89.74 & \ubold 46.87&76.66&81.12&81.47&81.74 & 28.48&67.19&72.30&72.88&73.34 \\
    \midrule
    MPNP-c   & \ubold 57.18&\ubold86.08&90.81&91.37&91.75 & 45.52&\ubold78.95&83.80&84.31&84.75 & \ubold31.52&\ubold74.30&81.38&82.20&82.64 \\
    \midrule
    \texttt{labelprop}     & 55.55&84.37&\ubold91.90&\ubold93.93&\ubold96.41 & 41.12&69.84&\ubold84.40&\ubold87.76&\ubold91.92 & 30.29&66.61&\ubold83.61&\ubold87.91&\ubold92.94 \\
    GCN      & 36.14 & 36.14 & 36.14 & 36.14 & 36.14 & 21.68 & 21.68 & 21.68 & 21.68 & 21.68 & 15.82 & 15.82 & 15.82 & 15.82 & 15.82 \\
    \bottomrule
  \end{tabular}}
\end{table*}

\begin{table}
    \centering
        \scriptsize
        \caption{Results on the Cora-Branched transductive learning tasks (mixed-class). Mean accuracy and standard deviations are reported at $\{1, 5, 10, 30\}$\% sampling rates.}
        \label{tab:cora_branched}
        \sisetup{%
            table-align-uncertainty=true,
            separate-uncertainty=true,
            detect-weight=true,
            detect-inline-weight=math,
            mode=text
        }
        \begin{tabular}{cl|*{5}{S[table-format=2.2]@{\,\(\tinypm \)\,}S[table-format=1.2]}}
            \toprule
            \% & Model & \multicolumn{2}{c}{2-class} & \multicolumn{2}{c}{3-class} & \multicolumn{2}{c}{5-class} & \multicolumn{2}{c}{7-class} & \multicolumn{2}{c}{11-class} \\
            \midrule \multirow{4}{*}{1} & NP-c & 77.99 & 1.11 & 67.00 & 1.83 & 60.47 & 0.69 & 52.83 & 0.49 & 34.57 & 2.18 \\
            & MPNP-c & \ubold 87.01 & \ubold 0.55 & \ubold 79.71 & \ubold 1.04 & \ubold 67.75 & \ubold 0.71 & \ubold 58.40 & \ubold 0.77 & 43.62& 1.01\\
            & \texttt{labelprop} & 74.84 & 0.44 & 65.31 & 0.73 & 56.41 & 0.26 & 52.62 & 0.31 & \ubold 46.84 & \ubold 0.55  \\
            & Mode & 68.62& 0.11& 54.35 & 0.10 & 38.86 & 0.14 & 30.48 & 0.16 & 21.60 & 0.08 \\
            
            \midrule \multirow{4}{*}{5} & NP-c & 87.16 & 0.59 & 76.99 & 1.50 & 70.51 & 0.40 & 63.02 & 0.50 & 37.94 & 0.84 \\
            & MPNP-c & \ubold 93.60 & \ubold 0.22 & \ubold 88.28 & \ubold 0.59 & \ubold 78.41 & \ubold 0.46 & \ubold 68.96& \ubold1.08& 50.64& 1.14\\
            & \texttt{labelprop} & 82.04 & 0.17 & 75.57 & 0.31 & 68.78 & 0.19 & 64.85& 0.22& \ubold 60.11& \ubold 0.12 \\
            & Mode & 68.84 & 0.22 & 54.28 & 0.07 & 38.84 & 0.07 & 30.57 & 0.07 & 21.60 & 0.11\\
            
            \midrule \multirow{4}{*}{10} & NP-c & 88.97 & 0.60 & 78.56 & 1.19 & 72.06 & 0.46 & 64.29 & 0.43 & 38.88 & 0.80 \\
            & MPNP-c & \ubold 94.40 & \ubold 0.17 & \ubold 89.41 & \ubold 0.58 & \ubold 79.70 & \ubold 0.65 & \ubold 70.53& \ubold 0.88 & 51.87& 1.23\\
            & \texttt{labelprop} & 83.81 & 0.07 & 77.90 & 0.16 & 72.07 & 0.13 & 68.55& 0.14& \ubold 64.22 & \ubold 0.08 \\
            & Mode & 68.51 & 0.16 & 54.40 & 0.27 & 38.93 & 0.12 & 30.50 & 0.10 & 21.63 & 0.09\\
            
            \midrule \multirow{4}{*}{30} & NP-c & 89.69 & 0.52 & 79.61 & 1.20 & 72.95 & 0.48 & 65.23 & 0.51 & 39.42 & 0.78 \\
            & MPNP-c & \ubold 94.77 & \ubold 0.19 & \ubold 90.02 & \ubold 0.60 & \ubold 80.52 & \ubold 0.62 & 71.54& 0.91& 52.67& 1.24\\
            & \texttt{labelprop} & 87.02 & 0.35 & 82.04& 0.18 & 77.56 & 0.11 & \ubold74.96 & \ubold0.20 & \ubold71.73 & \ubold0.05 \\
            & Mode & 68.46 & 0.11 & 54.41 & 0.18 & 38.81 & 0.12 & 30.50 & 0.10 & 21.66 & 0.10\\
            \bottomrule 
        \end{tabular}
\end{table}

\begin{table*}
  \scriptsize
  \caption{Performance on the Cora-Branched few-shot learning tasks. Accuracy at $\{1,5,10\}$\% context points.}
  \label{tab:fsl_cora}
  \centering
  \begin{tabular}{lccc|ccc|ccc|ccc}
    \toprule
    & \multicolumn{3}{c}{2-class} & \multicolumn{3}{c}{3-class} & \multicolumn{3}{c}{5-class} & \multicolumn{3}{c}{11-class}                  \\
    Model & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 \\
    \midrule
    NP-c     & 59.25&63.53&64.29 & 49.82&56.93&59.03 & 36.84&42.68&44.10 & 19.71&21.13&21.82 \\
    MPNP-c   & \ubold 62.91& \ubold67.53&\ubold68.57 &  \ubold 53.83&\ubold63.75&\ubold64.52 &  \ubold 41.67&\ubold49.99&\ubold51.15 & \ubold 23.56&\ubold26.00&\ubold27.44 \\
    \bottomrule
  \end{tabular}
\end{table*}



\begin{table}
    \centering
        \scriptsize
        \caption{Results on the Cora-Branched transductive learning tasks (mixed-class). Mean accuracy and standard deviations are reported at $\{1, 5, 10, 30\}$\% sampling rates.}
        \label{tab:cora_branched}
        \sisetup{%
            table-align-uncertainty=true,
            separate-uncertainty=true,
            detect-weight=true,
            detect-inline-weight=math,
            mode=text
        }
        % \begin{adjustbox}{width=1.0\columnwidth}
        \begin{tabular}{cl|*{5}{S[table-format=2.2]@{\,\(\tinypm \)\,}S[table-format=1.2]}}
            \toprule
            \% & Model & \multicolumn{2}{c}{3-class} & \multicolumn{2}{c}{7-class} & \multicolumn{2}{c}{11-class} \\
            \midrule \multirow{4}{*}{1} & NP-c & 67.00 & 1.83 & 52.83 & 0.49 & 34.57 & 2.18 \\
            & MPNP-c & \ubold 79.71 & \ubold 1.04 & \ubold 58.40 & \ubold 0.77 & 43.62& 1.01\\
            & \texttt{labelprop} & 65.31 & 0.73 & 52.62 & 0.31 & \ubold 46.84 & \ubold 0.55  \\
            & Mode & 54.35 & 0.10 & 30.48 & 0.16 & 21.60 & 0.08 \\
            
            \midrule \multirow{4}{*}{5} & NP-c & 76.99 & 1.50 & 63.02 & 0.50 & 37.94 & 0.84 \\
            & MPNP-c & \ubold 88.28 & \ubold 0.59 & \ubold 68.96& \ubold1.08& 50.64& 1.14\\
            & \texttt{labelprop} & 75.57 & 0.31 & 64.85& 0.22& \ubold 60.11& \ubold 0.12 \\
            & Mode & 54.28 & 0.07 & 30.57 & 0.07 & 21.60 & 0.11\\
            
            \midrule \multirow{4}{*}{10} & NP-c & 78.56 & 1.19 & 64.29 & 0.43 & 38.88 & 0.80 \\
            & MPNP-c & \ubold 89.41 & \ubold 0.58 &\ubold 70.53& \ubold 0.88 & 51.87& 1.23\\
            & \texttt{labelprop} & 77.90 & 0.16 & 68.55& 0.14& \ubold 64.22 & \ubold 0.08 \\
            & Mode & 54.40 & 0.27 & 30.50 & 0.10 & 21.63 & 0.09\\
            
            \midrule \multirow{4}{*}{30} & NP-c & 79.61 & 1.20 & 65.23 & 0.51 & 39.42 & 0.78 \\
            & MPNP-c & \ubold 90.02 & \ubold 0.60 & 71.54& 0.91& 52.67& 1.24\\
            & \texttt{labelprop} & 82.04& 0.18 & \ubold74.96 & \ubold0.20 & \ubold71.73 & \ubold0.05 \\
            & Mode & 54.41 & 0.18 & 30.50 & 0.10 & 21.66 & 0.10\\
            \bottomrule 
        \end{tabular}
        % \end{adjustbox}
\end{table}

\begin{table}
  \scriptsize
  \caption{Performance on the Cora-Branched few-shot learning tasks. Accuracy at $\{1,5,10\}$\% context points.}
  \label{tab:fsl_cora}
  \centering
  \begin{tabular}{clcccc}
    \toprule
    \% & Model & 2-class & 3-class & 5-class & 11-class \\
    \midrule
    \multirow{2}{*}{1}
    & NP-C   & 59.25 & 49.82 & 36.84 & 19.71 \\
    & MPNP-C & \ubold 62.91 & \ubold 53.83 & \ubold 41.67 & \ubold 23.56 \\
    \midrule
    \multirow{2}{*}{5}
    & NP-C   & 63.53 & 56.93 & 42.68 & 21.13 \\
    & MPNP-C & \ubold 67.53 & \ubold 63.75 & \ubold 49.99 & \ubold 26.00 \\
    \midrule
    \multirow{2}{*}{10}
    & NP-C   & 64.29 & 59.03 & 44.10 & 21.82 \\
    & MPNP-C & \ubold 68.57 & \ubold 64.52 & \ubold 51.15 & \ubold 27.44 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}
    \scriptsize
    \centering
    % \begin{adjustbox}{width=1.0\columnwidth}
    \begin{tabular}{clccr}
        \toprule
        \% & Model & 2-class & 3-class & 4-class \\
        \midrule \multirow{4}{*}{0.1}
        &	 NP-C	 &	 48.06	 &	  \ubold 46.87	 &	 28.48 \\
        &	 MPNP-C	 &	 \ubold 57.18	 &	 45.52	 &	  \ubold  31.52 \\
        & \texttt{labelprop} &	 55.55	 &	 41.12	 &	 30.29 \\
        & GCN   &	 36.14	 &	 21.68	 & 15.82 \\
        \midrule \multirow{4}{*}{1}
        &	 NP-C	 &	 83.60	 &	 76.66	 &	 67.19 \\
        &	 MPNP-C	 &	  \ubold  86.08	 &	  \ubold  78.95	 &	 \ubold   74.30 \\
        & \texttt{labelprop}  &	 84.37	 &	 69.84	 &	 66.61 \\
        &	 GCN	&	 36.14	 &	 21.68	 &	 15.82 \\
        \midrule \multirow{4}{*}{5}
        &	 NP-C	 &	 88.61	 &	 81.12	 &	 72.30 \\
        &	 MPNP-C	 &	 90.81	 &	 83.80	 &	 81.38 \\
        &	 \texttt{labelprop}	 &	  \ubold  91.90	 &	  \ubold 84.40	 &	 \ubold  83.61 \\
        &	 GCN 	 &	 36.14	 &	 21.68	 &	 15.82 \\
        \midrule \multirow{4}{*}{10}
        &	 NP-C	 &	 89.17	 &	 81.47	 &	 72.88 \\
        &	 MPNP-C	 &	 91.37	 &	 84.31	 &	 82.20 \\
        &	 \texttt{labelprop}	 &	  \ubold 93.93	 &	  \ubold 87.76	 &	  \ubold  87.91 \\
        &	 GCN 	 &	 36.14	 &	 21.68	 &	 15.82 \\
        \bottomrule
    \end{tabular}
    % \end{adjustbox}
    \caption{ShapeNet mixed-class results. We report the mIoU for $\{0.1, 1, 5, 10\}$\% context points.}
    \label{tab:my_label}
\end{table}
